O(a) improvement of the HYP static axial and vector currents at one-loop order of perturbation theory

We calculate analytically the improvement coefficients of the static axial and vector currents in O(a) improved lattice QCD at one-loop order of perturbation theory. The static quark is described by the hypercubic action, previously introduced in the literature in order to improve the signal-to-noise ratio of static observables. Within a Schroedinger Functional setup, we derive the Feynman rules of the hypercubic link in time-momentum representation. The improvement coefficients are obtained from on-shell correlators of the static axial and vector currents. As a by-product, we localise the minimum of the static self-energy as a function of the smearing parameters of the action at one-loop order and show that the perturbative minimum is close to its non-perturbative counterpart.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CUSTOM COMMANDS


% Abbreviations for environment tags
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}

% References
\newcommand{\req}[1]{Eq.~(\ref{#1})}
\newcommand{\res}[1]{Section~\ref{#1}}
\newcommand{\reapp}[1]{Appendix~\ref{#1}}
\newcommand{\rep}[1]{\cite{#1}}
\newcommand{\refig}[1]{Fig.~\ref{#1}}
\newcommand{\ret}[1]{Table~\ref{#1}}

% Miscellaneous symbols
\newcommand{\dif}{{\rm d}}
\newcommand{\Tr}{{\rm Tr}}
\newcommand{\tr}{{\rm tr}}
\newcommand{\Pf}{{\rm Pf}}
\newcommand{\Id}{\mathbf{1}}
\newcommand{\pexp}{\mbox{P} \, \mbox{exp}}
\newcommand{\Per}[1]{\mathbf{S}_{#1}}
\newcommand{\eps}{\varepsilon}
\newcommand{\ci}[1]{\boldsymbol{#1}}
\renewcommand{\Re}[1]{{\mathcal Re}\left\{#1\right\}}
\renewcommand{\Im}[1]{{\mathcal Im}\left\{#1\right\}}
\newcommand{\Dslash}{\relax{\kern+.25em / \kern-.70em D}}
\newcommand{\Dwd}{D_{\rm\scriptstyle w}}
\newcommand{\Dtwd}{D_{\rm\scriptstyle tw}}
\newcommand{\arcsinh}{\rm arcsinh}
\newcommand{\arccosh}{\rm arccosh}
\newcommand{\arctanh}{\rm arctanh}
\newcommand{\fm}{{\rm fm}}
\newcommand{\MeV}{{\rm MeV}}
\newcommand{\GeV}{{\rm GeV}}

% Numerical sets / Groups
\newcommand{\Real}{\relax{\mathsf{\Gamma\kern-.35em R}}}
\newcommand{\Int}{\relax{\mathsf{Z\kern-.40em Z}}}
\newcommand{\Ztwo}{Z_2}
\newcommand{\Zf}{Z_4}
\newcommand{\ZN}{Z_{\NC}}
\newcommand{\ZTN}{Z_{2\NC}}
\newcommand{\UO}{\mbox{U}(1)}
\newcommand{\SUT}{\mbox{SU}(2)}
\newcommand{\UT}{\mbox{U}(2)}
\newcommand{\SUt}{\mbox{SU}(3)}
\newcommand{\Ut}{\mbox{U}(3)}
\newcommand{\SUN}{\mbox{SU}(\NC)}
\newcommand{\UN}{\mbox{U}(\NC)}
\newcommand{\SUQ}{\mbox{SU}(Q)}
\newcommand{\UQ}{\mbox{U}(Q)}
\newcommand{\SU}{\mbox{SU}}
\newcommand{\CF}{C_{\rm F}}

% Scriptstyle fractions
\newcommand{\half}{{\scriptstyle{{1\over 2}}}}
\newcommand{\third}{{\scriptstyle{{1\over 3}}}}
\newcommand{\quart}{{\scriptstyle{{1\over 4}}}}
\newcommand{\sixth}{{\scriptstyle{{1\over 6}}}}
\newcommand{\eighth}{{\scriptstyle{{1\over 8}}}}
\newcommand{\sixteenth}{{\scriptstyle{{1\over 16}}}}
\newcommand{\twth}{{\scriptstyle{{1\over 12}}}}
\newcommand{\thalf}{{\scriptstyle{{3\over 2}}}}
\newcommand{\fhalf}{{\scriptstyle{{5\over 2}}}}
\newcommand{\tthird}{{\scriptstyle{{2\over 3}}}}
\newcommand{\fthird}{{\scriptstyle{{5\over 3}}}}
\newcommand{\ihalf}{{\scriptstyle{{i\over 2}}}}
\newcommand{\iquart}{{\scriptstyle{{i\over 4}}}}
\newcommand{\oneovN}{{\scriptstyle{{1\over \NC}}}}

% Colours, flavours, susies
%\newcommand{\NC}{N_c}
\newcommand{\NC}{N}
\newcommand{\NF}{N_\mathrm{\scriptstyle f}}
\newcommand{\NSS}{{\cal N}}

% Renormalisation schemes
\newcommand{\MS}{{\rm MS}}
\newcommand{\MSbar}{{\overline{\rm MS}}}
\newcommand{\SF}{{\rm SF}}

% Renormalised, RGI and related quantities
\newcommand{\gbar}{\kern1pt\overline{\kern-1pt g\kern-0pt}\kern1pt}
\newcommand{\mbar}{\kern2pt\overline{\kern-1pt m\kern-1pt}\kern1pt}
\newcommand{\obar}[1]{\kern3pt\overline{\kern-2pt #1\kern-0pt}\kern1pt}
\newcommand{\gren}{g_{\rm R}}
\newcommand{\mren}[1]{m_{{\rm R} #1}}
\newcommand{\muren}[1]{\mu_{{\rm R} #1}}
\newcommand{\oren}[1]{#1_{\rm R}}
\newcommand{\lQCD}{\Lambda_{\rm\scriptscriptstyle QCD}}
\newcommand{\mrgi}{M}
\newcommand{\orgi}[1]{\hat #1}
\newcommand{\msubt}{m_{\rm q}}
\newcommand{\mcrit}{m_{\rm cr}}
\newcommand{\hopc}{\kappa_{\rm cr}}
\newcommand{\muq}{\mu_{\rm q}}

% Correlation functions
\newcommand{\fX}{f_{\rm\scriptscriptstyle X}}
\newcommand{\fP}{f_{\rm\scriptscriptstyle P}}
\newcommand{\fS}{f_{\rm\scriptscriptstyle S}}
\newcommand{\fA}{f_{\rm\scriptscriptstyle A}}
\newcommand{\fV}{f_{\rm\scriptscriptstyle V}}
\newcommand{\kX}{k_{\rm\scriptscriptstyle X}}
\newcommand{\kA}{k_{\rm\scriptscriptstyle A}}
\newcommand{\kV}{k_{\rm\scriptscriptstyle V}}
\newcommand{\kT}{k_{\rm\scriptscriptstyle T}}
\newcommand{\hT}{h_{\rm\scriptscriptstyle T}}

% Z's, SSF's et rel.
\newcommand{\Zm}{Z_{\rm m}}
\newcommand{\ZP}{Z_{\rm\scriptscriptstyle P}}
\newcommand{\ZS}{Z_{\rm\scriptscriptstyle S}}
\newcommand{\ZA}{Z_{\rm\scriptscriptstyle A}}
\newcommand{\ZV}{Z_{\rm\scriptscriptstyle V}}
\newcommand{\ZT}{Z_{\rm\scriptscriptstyle T}}
\newcommand{\sigmaP}{\sigma_{\rm\scriptscriptstyle P}}
\newcommand{\sigmaT}{\sigma_{\rm\scriptscriptstyle T}}
\newcommand{\SigmaP}{\Sigma_{\rm\scriptscriptstyle P}}
\newcommand{\SigmaT}{\Sigma_{\rm\scriptscriptstyle T}}
\newcommand{\lmax}{L_{\rm max}}
\newcommand{\lmin}{L_{\rm min}}

% O(a) improvement
\newcommand{\Oa}{\mbox{O}(a)}
\newcommand{\Oasq}{\mbox{O}(a^2)}
\newcommand{\Ogsqa}{\mbox{O}(g_0^2 a)}
\newcommand{\Ogqa}{\mbox{O}(g_0^4 a)}
\newcommand{\icsw}{c_{\rm sw}}
\newcommand{\ict}{c_{\rm t}}
\newcommand{\icttil}{\tilde c_{\rm t}}
\newcommand{\icP}{c_{\rm\scriptscriptstyle P}}
\newcommand{\icA}{c_{\rm\scriptscriptstyle A}}
\newcommand{\icT}{c_{\rm\scriptscriptstyle T}}
\newcommand{\icV}{c_{\rm\scriptscriptstyle V}}
\newcommand{\ibP}{b_{\rm\scriptscriptstyle P}}
\newcommand{\ibA}{b_{\rm\scriptscriptstyle A}}
\newcommand{\ibT}{b_{\rm\scriptscriptstyle T}}
\newcommand{\ibV}{b_{\rm\scriptscriptstyle V}}
\newcommand{\ibm}{b_{\rm m}}
\newcommand{\ibmtil}{\tilde{b}_{\rm m}}
\newcommand{\ibmu}{b_\mu}

% Ginsparg-Wilson
\newcommand{\abar}{\kern1pt\overline{\kern-1pt a\kern-0.5pt}\kern1pt}
\newcommand{\abarhalf}{{\scriptstyle \frac{\abar}{2}}}
\newcommand{\psil}{\psi_{\mbox{\tiny L}}}

% Boldface and calligraphic capitals
\newcommand{\bA}{{\mathbf{A}}}
\newcommand{\bB}{{\mathbf{B}}}
\newcommand{\bC}{{\mathbf{C}}}
\newcommand{\bD}{{\mathbf{D}}}
\newcommand{\bE}{{\mathbf{E}}}
\newcommand{\bF}{{\mathbf{F}}}
\newcommand{\bG}{{\mathbf{G}}}
\newcommand{\bH}{{\mathbf{H}}}
\newcommand{\bI}{{\mathbf{I}}}
\newcommand{\bJ}{{\mathbf{J}}}
\newcommand{\bK}{{\mathbf{K}}}
\newcommand{\bL}{{\mathbf{L}}}
\newcommand{\bM}{{\mathbf{M}}}
\newcommand{\bN}{{\mathbf{N}}}
\newcommand{\bO}{{\mathbf{O}}}
\newcommand{\bP}{{\mathbf{P}}}
\newcommand{\bQ}{{\mathbf{Q}}}
\newcommand{\bR}{{\mathbf{R}}}
\newcommand{\bS}{{\mathbf{S}}}
\newcommand{\bT}{{\mathbf{T}}}
\newcommand{\bU}{{\mathbf{U}}}
\newcommand{\bV}{{\mathbf{V}}}
\newcommand{\bW}{{\mathbf{W}}}
\newcommand{\bX}{{\mathbf{X}}}
\newcommand{\bY}{{\mathbf{Y}}}
\newcommand{\bZ}{{\mathbf{Z}}}
\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cI}{{\cal I}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cQ}{{\cal Q}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cY}{{\cal Y}}
\newcommand{\cZ}{{\cal Z}}

% Boldface three-vectors and funny caps for momenta
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\vt}{\mathbf{t}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vq}{\mathbf{q}}
\newcommand{\vk}{\mathbf{k}}
\newcommand{\vl}{\mathbf{l}}
\newcommand{\vn}{\mathbf{n}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\vzero}{\mathbf{0}}
\newcommand{\ring}[1]{\mathaccent"7017 #1}

\newcommand{\heavy}{\psi_{\rm \phantom{\bar{h}^\dagger}\hspace{-0.28cm}h}}
\newcommand{\heavyb}{{\bar{\psi}}_{\rm h}}
\newcommand{\aheavy}{\psi_{{\rm \phantom{\bar{h}^\dagger}\hspace{-0.28cm}\bar{h}}}}
\newcommand{\aheavyb}{\bar{\psi}_{\bar{\rm h}}}

\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\by}{{\mathbf{y}}}

\newcommand{\parbreak}{\vskip 0.2cm}

\newcommand{\cAstat}{{c^{\rm stat}_{\rm\scriptscriptstyle A}}}
\newcommand{\bAstat}{{b^{\rm stat}_{\rm\scriptscriptstyle A}}}
\newcommand{\cVstat}{{c^{\rm stat}_{\rm\scriptscriptstyle V}}}
\newcommand{\bVstat}{{b^{\rm stat}_{\rm\scriptscriptstyle V}}}

